Convolution-t Distributions

We introduce a new class of multivariate heavy-tailed distributions that are convolutions of heterogeneous multivariate t-distributions. Unlike commonly used heavy-tailed distributions, the multivariate convolution-t distributions embody cluster structures with flexible nonlinear dependencies and heterogeneous marginal distributions. Importantly, convolution-t distributions have simple density functions that facilitate estimation and likelihood-based inference. The characteristic features of convolution-t distributions are found to be important in an empirical analysis of realized volatility measures and help identify their underlying factor structure.

==> Tables/Table1.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{0.7cm}YYYp{0cm}YYYp{0cm}YYYYYY}
\toprule
\midrule
          & \multicolumn{3}{c}{Energe} &       & \multicolumn{3}{c}{Health Care} &       & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule{2-4}\cmidrule{6-8}\cmidrule{10-12}          & CVX   & MRO   & OXY   &       & JNJ   & LLY   & MRK   &       & AAPL  & MU    & ORCL \\
\midrule          
          &       &       &       &       &       &       &       &       &       &       &  \\
    $\xi$ & -0.517 & -0.342 & -0.362 &       & -0.653 & -0.609 & -0.652 &       & -0.360 & -0.391 & -0.524 \\
          & \textit{(0.085)} & \textit{(0.070)} & \textit{(0.073)} &       & \textit{(0.106)} & \textit{(0.103)} & \textit{(0.103)} &       & \textit{(0.073)} & \textit{(0.077)} & \textit{(0.089)} \\
\\[-0.2cm]
    $\beta_d$ & 0.483 & 0.448 & 0.431 &       & 0.410 & 0.401 & 0.438 &       & 0.453 & 0.438 & 0.423 \\
          & \textit{(0.017)} & \textit{(0.017)} & \textit{(0.017)} &       & \textit{(0.017)} & \textit{(0.017)} & \textit{(0.017)} &       & \textit{(0.017)} & \textit{(0.017)} & \textit{(0.017)} \\
\\[-0.2cm]
    $\beta_w$ & 0.348 & 0.357 & 0.374 &       & 0.324 & 0.340 & 0.325 &       & 0.320 & 0.320 & 0.361 \\
          & \textit{(0.026)} & \textit{(0.027)} & \textit{(0.027)} &       & \textit{(0.028)} & \textit{(0.028)} & \textit{(0.027)} &       & \textit{(0.027)} & \textit{(0.027)} & \textit{(0.027)} \\
\\[-0.2cm]
    $\beta_m$ & 0.113 & 0.153 & 0.152 &       & 0.194 & 0.193 & 0.165 &       & 0.186 & 0.198 & 0.158 \\
          & \textit{(0.021)} & \textit{(0.022)} & \textit{(0.022)} &       & \textit{(0.025)} & \textit{(0.024)} & \textit{(0.023)} &       & \textit{(0.022)} & \textit{(0.023)} & \textit{(0.022)} \\
          &       &       &       &       &       &       &       &       &       &       &  \\

    $\mathbb{E}(Y)$  & -9.097 & -8.179 & -8.546 &       & -9.156 & -9.130 & -9.133 &       & -8.830 & -8.703 & -9.062  \\
    $\pi$    & 0.943 & 0.958 & 0.958 &       & 0.929 & 0.933 & 0.929 &       & 0.959 & 0.955 & 0.942  \\
 
    $\sigma_v$ & 0.480 & 0.478 & 0.492 &       & 0.539 & 0.552 & 0.521 &       & 0.502 & 0.497 & 0.524 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table2.tex <==
\vspace{0.2cm}
\begin{small}
%\begin{tabular}{p{0.3cm}  p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} }
\begin{tabularx}{\textwidth}{XXYYYYYYYYY}
\toprule
\midrule
  & &  \multicolumn{3}{c}{Energy} & \multicolumn{3}{c}{Health Care} & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule(l){3-5}
\cmidrule(l){6-8}
\cmidrule(l){9-11}
  &  & CVX & MRO & OXY   & JNJ   & LLY   & MRK & AAPL & MU & ORCL \\
\midrule
% & & \multicolumn{9}{c}{\textit{Panel A: Correlation Matrix and Its logarithm}} \\
\\[-0.1cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize Energy}}} & CVX & 1.000 &  0.561 &  0.580 & \cellcolor{black!10}0.303 & \cellcolor{black!10}0.323 & \cellcolor{black!10}0.316 &  0.375 &  0.361 &  0.367 \\
  &  &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &   &  
\\[-0.1cm]
  & MRO & 0.561 & 1.000 & 0.557 & \cellcolor{black!10}0.229 & \cellcolor{black!10}0.214 & \cellcolor{black!10}0.228 &  0.293 &  0.275 &  0.288 \\
  &  &   & &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &   &    & 
\\[-0.1cm]
  & OXY &  0.580 &  0.557 & 1.000 & \cellcolor{black!10}0.249 & \cellcolor{black!10}0.257 & \cellcolor{black!10}0.261 &   0.299 &  0.300 &  0.299 \\
\\[-0.1cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize Health Care}}} & JNJ & \cellcolor{black!10}0.303 & \cellcolor{black!10}0.229 & \cellcolor{black!10}0.249 & 1.000 &  0.427 &  0.407 & \cellcolor{black!10}0.304 & \cellcolor{black!10}0.260 & \cellcolor{black!10}0.326 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.1cm]
  & LLY & \cellcolor{black!10}0.323 & \cellcolor{black!10}0.214 & \cellcolor{black!10}0.257 &  0.427 & 1.000 &  0.474 & \cellcolor{black!10}0.307 & \cellcolor{black!10}0.265 & \cellcolor{black!10}0.310 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.1cm]
  & MRK & \cellcolor{black!10}0.316 & \cellcolor{black!10}0.228 & \cellcolor{black!10}0.261 &  0.407 &  0.474 &  1.000 & \cellcolor{black!10}0.316 & \cellcolor{black!10}0.290 & \cellcolor{black!10}0.307 \\
\\[-0.1cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize Info Tech.}}} & AAPL & 0.375 & 0.293 & 0.299& \cellcolor{black!10}0.304 & \cellcolor{black!10}0.307 & \cellcolor{black!10}0.316 & 1.000 &  0.463 &  0.459 \\
  &  &  &   &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  & 
\\[-0.1cm]
  & MU &  0.361 & 0.275 & 0.300 & \cellcolor{black!10} 0.260 & \cellcolor{black!10} 0.265 & \cellcolor{black!10} 0.290 & 0.463 & 1.000 & 0.439 \\
  &  &   &   &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  & & 
\\[-0.1cm]
  & ORCL &  0.367 & 0.288 & 0.299 & \cellcolor{black!10} 0.326 & \cellcolor{black!10} 0.310 & \cellcolor{black!10} 0.307 & 0.459 & 0.439 & 1.000  \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table3.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{2.0cm}YYYYYYYYYYYYY}
\toprule
\midrule
          & {Gaussian} & {Multivariate $t$} & {Conv-$t$ (Sector)} & {Conv-$t$ (Hetero)} \\
    \midrule
          &       &       &       &  \\          
    $\nu_{(\text{Joint})}$ & $\infty$       & 10.717 &   &  \\
          &       & \textit{(0.379)} &                \\
          &       &       &       & \cellcolor{black!10}9.963  \\
          &       &       &       & \cellcolor{black!10} \textit{(1.259)}  \\
    $\nu_{(\text{Energy})}$ &       &       &  8.474 & \cellcolor{black!10} 7.294  \\
          &       &       & \textit{(0.457)} & \cellcolor{black!10} \textit{(0.643)} \\
          &       &       &       & \cellcolor{black!10} 7.103  \\
          &       &       &       & \cellcolor{black!10} \textit{(0.605)}  \\
          &       &       &       &  \cellcolor{black!5}5.653  \\
          &       &       &       &  \cellcolor{black!5} \textit{(0.354)}   \\
    $\nu_{(\text{Health Care})}$ &       &       & 6.311 & \cellcolor{black!5} 5.342  \\
          &       &       & \textit{(0.234)} & \cellcolor{black!5} \textit{(0.298)} \\
          &       &       &       & \cellcolor{black!5} 5.969  \\
          &       &       &       & \cellcolor{black!5} \textit{(0.394)}  \\
          &       &       &       & \cellcolor{black!10}8.665  \\
          &       &       &       & \cellcolor{black!10}\textit{(0.936)} \\
     $\nu_{(\text{Info Tech.})}$ &       &       & 9.203 & \cellcolor{black!10}8.197 \\
          &       &       & \textit{(0.535)} & \cellcolor{black!10}\textit{(0.873)}  \\
          &       &       &       & \cellcolor{black!10}8.750  \\
          &       &       &       & \cellcolor{black!10} \textit{(0.889)}  \\          
          \\[0.0cm]
    $\ell$   & -26,721 & -25,783 & \textbf{-25,578} & -25,700 \\
    $\ell_m$ & -33,149 & -32,457 & -32,403 & \textbf{-32,398} \\
    $\ell_c$ & 6,428  & 6,674  & \textbf{6,825} & 6,699 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table32.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{2.0cm}Yp{0.3cm}Yp{0.3cm}YYp{0.3cm}YY}
    \toprule
          & {Gaussian} &       & {Multi-$t$} &       & \multicolumn{2}{c}{Conv-$t$ (Sector)} &       & \multicolumn{2}{c}{Conv-$t$ (Hetero)} \\
          &       &       &       &       & sym   & asym  &       & sym   & asym \\
    \midrule
          &       &       &       &       &       &       &       &       &  \\
    $\nu_{(\text{Joint})}$    & $\infty$      &       & 10.717 &       &       &       &       &       &  \\
          &       &       & \textit{(0.379)} &       &       &       &       &       &  \\
          &       &       &       &       &       &       &       & 9.963 & 7.531 \\
          &       &       &       &       &       &       &       & \textit{(1.259)} & \textit{(0.712)} \\
    $\nu_{(\text{Energy})}$    &       &       &       &       & 8.474 & 8.068 &       & 7.294 & 5.549 \\
          &       &       &       &       & \textit{(0.457)} & \textit{(0.466)} &       & \textit{(0.643)} & \textit{(0.396)} \\
          &       &       &       &       &       &       &       & 7.103 & 6.719 \\
          &       &       &       &       &       &       &       & \textit{(0.605)} & \textit{(0.682)} \\
          &       &       &       &       &       &       &       & 5.653 & 5.328 \\
          &       &       &       &       &       &       &       & \textit{(0.354)} & \textit{(0.306)} \\
    $\nu_{(\text{Health Care})}$    &       &       &       &       & 6.311 & 6.150 &       & 5.342 & 5.184 \\
          &       &       &       &       & \textit{(0.234)} & \textit{(0.242)} &       & \textit{(0.298)} & \textit{(0.279)} \\
          &       &       &       &       &       &       &       & 5.969 & 5.659 \\
          &       &       &       &       &       &       &       & \textit{(0.394)} & \textit{(0.393)} \\
          &       &       &       &       &       &       &       & 8.665 & 11.919 \\
          &       &       &       &       &       &       &       & \textit{(0.936)} & \textit{(3.459)} \\
    $\nu_{(\text{Info Tech.})}$    &       &       &       &       & 9.203 & 8.864 &       & 8.197 & 6.546 \\
          &       &       &       &       & \textit{(0.535)} & \textit{(0.529)} &       & \textit{(0.873)} & \textit{(0.560)} \\
          &       &       &       &       &       &       &       & 8.750 & 7.011 \\
          &       &       &       &       &       &       &       & \textit{(0.889)} & \textit{(0.650)} \\
          &       &       &       &       &       &       &       &       &  \\
    $p$     & 0     &       & 1     &       & 3     & 39    &       & 9 & 45 \\
          &       &       &       &       &       &       &       &       &  \\
    $\ell$   & -26721 &       & -25783 &       & -25578 & -25482 &       & -25700 & \textbf{-25463} \\
    $\ell_m$ & -33149 &       & -32457 &       & -32403 & -32426 &       & \textbf{-32398} & -32419 \\
    $\ell_c$ & 6428  &       & 6674  &       & 6825  & 6944  &       & 6699  & \textbf{6955} \\
          &       &       &       &       &       &       &       &       &  \\
    BIC   & 53442 &       & 51575 &       & \textbf{51182} & 51296 &       & 51477 & 51309 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table4.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{1.8cm}YYYp{-0.5cm}YYYp{-0.5cm}YYYYYY}
\toprule
\midrule
          & \multicolumn{3}{c}{Energe} &       & \multicolumn{3}{c}{Health Care} &       & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule{2-4}\cmidrule{6-8}\cmidrule{10-12}          & CVX   & MRO   & OXY   &       & JNJ   & LLY   & MRK   &       & AAPL  & MU    & ORCL \\
\midrule          
          &       &       &       &       &       &       &       &       &       &       &  \\
 %Empirical & 1.103 & 1.211 & 1.528 &       & 2.325 & 2.972  &  2.076 &       & 0.902 &   0.996  &  0.993 \\  
%\\[-0.2cm]   
   Student's-$t$ & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893  \\
\\[-0.2cm]
   Group-$t$ &  1.114 & 1.230 & 1.207 &       & 2.339 & 2.346 & 2.325 &       & 0.998 & 1.023 & 0.999 \\
\\[-0.2cm]
   Hetero-$t$ & 0.638 & 1.285 & 1.334 &       & 2.865 & 3.443 & 2.321 &       & 0.940 & 1.079 & 0.945 \\ 
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table41.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{2.3cm}YYYp{-0.5cm}YYYp{-0.5cm}YYYYYY}
\toprule
\midrule
          & \multicolumn{3}{c}{Energe} &       & \multicolumn{3}{c}{Health Care} &       & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule{2-4}\cmidrule{6-8}\cmidrule{10-12}          & CVX   & MRO   & OXY   &       & JNJ   & LLY   & MRK   &       & AAPL  & MU    & ORCL \\
\midrule          
\\[0.0cm] 
 %Empirical & 1.103 & 1.211 & 1.528 &       & 2.325 & 2.972  &  2.076 &       & 0.902 &   0.996  &  0.993 \\  
   $t$-QMLE $(Y_t)$ & 0.890 & 0.888 & 1.037 &       & 2.455 & 3.103 & 2.206 &       & 0.902 & 0.996 & 0.993  \\
\\[-0.2cm]   
   $t$-QMLE  $(\hat{U}_t)$ & 1.006 & 1.811 & 1.877 &       & 3.748 & 4.271 & 2.940 &       & 1.272 & 1.372 & 1.266 \\    
\\[0.0cm]    
\multicolumn{12}{l}{\it Panel A: Conditional Excess Kurtosis for $Y_t$ }   \\
\\[-0.2cm] 
   Student's-$t$ & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893  \\
\\[-0.2cm]
   Group-$t$ &  1.114 & 1.230 & 1.207 &       & 2.339 & 2.346 & 2.325 &       & 0.998 & 1.023 & 0.999 \\
\\[-0.2cm]
   Hetero-$t$ & 0.638 & 1.285 & 1.334 &       & 2.865 & 3.443 & 2.321 &       & 0.940 & 1.079 & 0.945 \\
\\[0.0cm]
\multicolumn{12}{l}{\it Panel B: Excess Kurtosis for $\hat{U}_t$ }   \\
\\[-0.2cm] 
   Student's-$t$ & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893  \\
\\[-0.2cm]
   Group-$t$ &      1.341 & 1.341 & 1.341 &       & 2.596 & 2.596 & 2.596 &       & 1.153 & 1.153 & 1.153 \\
\\[-0.2cm]
   Hetero-$t$ & 1.006 & 1.821 & 1.934 &       & 3.629 & 4.470 & 3.047 &       & 1.286 & 1.430 & 1.263 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table42.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{2.5cm}YYYp{-0.5cm}YYYp{-0.5cm}YYYYYY}
\toprule
\midrule
          & \multicolumn{3}{c}{Energe} &       & \multicolumn{3}{c}{Health Care} &       & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule{2-4}\cmidrule{6-8}\cmidrule{10-12}          & CVX   & MRO   & OXY   &       & JNJ   & LLY   & MRK   &       & AAPL  & MU    & ORCL \\
\midrule          
\\[0.0cm]   
   $t$-QMLE $(Y_t)$ & 0.890 & 0.888 & 1.037 &       & 2.455 & 3.103 & 2.206 &       & 0.902 & 0.996 & 0.993  \\
\\[-0.2cm]   
   $t$-QMLE  $(\hat{U}_t)$ & 1.006 & 1.811 & 1.877 &       & 3.748 & 4.271 & 2.940 &       & 1.272 & 1.372 & 1.266 \\    
\\[0.0cm]    
\multicolumn{12}{l}{\it Panel A: Conditional Excess Kurtosis for $Y_t$ }   \\
\\[-0.2cm]
   Student's-$t$ & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893  \\
\\[-0.2cm]
   Group-$t$ (sym) &  1.114 & 1.230 & 1.207 &       & 2.339 & 2.346 & 2.325 &       & 0.998 & 1.023 & 0.999 \\
\\[-0.2cm]
   Group-$t$ (asym) &  0.814 & 1.017 & 1.135 &       & 1.586 & 1.641 & 1.565 &       & 0.664 & 0.663 & 0.670 \\
\\[-0.2cm]
   Hetero-$t$ (sym) & 0.638 & 1.285 & 1.334 &       & 2.865 & 3.443 & 2.321 &       & 0.940 & 1.079 & 0.945 \\
\\[-0.2cm]
   Hetero-$t$ (asym) & 0.638 & 0.943 & 0.727 &       & 2.247 & 2.546 & 1.894 &       & 0.546 & 0.883 & 0.814 \\   
\\[0.0cm]
\multicolumn{12}{l}{\it Panel B: Excess Kurtosis for $\hat{U}_t$ }   \\
\\[-0.2cm] 
   Student's-$t$ & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893 &       & 0.893 & 0.893 & 0.893  \\
\\[-0.2cm]
   Group-$t$ (sym)&      1.341 & 1.341 & 1.341 &       & 2.596 & 2.596 & 2.596 &       & 1.153 & 1.153 & 1.153 \\
\\[-0.2cm]
   Group-$t$ (asym)&      1.475 & 1.475 & 1.475 &       & 2.791 & 2.791 & 2.791 &       & 1.234 & 1.234 & 1.234 \\
\\[-0.2cm]
   Hetero-$t$ (sym) & 1.006 & 1.821 & 1.934 &       & 3.629 & 4.470 & 3.047 &       & 1.286 & 1.430 & 1.263 \\
\\[-0.2cm]
   Hetero-$t$ (asym) & 1.699 & 3.873 & 2.206 &       & 4.519 & 5.069 & 3.616 &       & 0.758 & 2.357 & 1.993 \\   
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table5.tex <==
\vspace{0.2cm}
\begin{small}
%\begin{tabular}{p{0.3cm}  p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} }
\begin{tabularx}{\textwidth}{m{0.5cm}XYYYYYYYYY}
\toprule
\midrule
  & &  \multicolumn{3}{c}{Energy} & \multicolumn{3}{c}{Health Care} & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule(l){3-5}
\cmidrule(l){6-8}
\cmidrule(l){9-11}
  &  & CVX & MRO & OXY   & JNJ   & LLY   & MRK & AAPL & MU & ORCL \\
\midrule
 & & \multicolumn{9}{c}{\textit{Panel A: Symmetric $B^\prime$ Matrix from $\hat{\Sigma}^{\frac{1}{2}}$}} \\
\\[-0.2cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad  Energy}}} & CVX & 0.425 & 0.116 & 0.122 & \cellcolor{black!10}0.052 & \cellcolor{black!10}0.058 & \cellcolor{black!10}0.053 & 0.065 & 0.062 & 0.064 \\
  &  &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &   &  
\\[-0.25cm]
  & MRO & 0.116 & 0.437 & 0.119 & \cellcolor{black!10}0.037 & \cellcolor{black!10}0.031 & \cellcolor{black!10}0.034 & 0.047 & 0.043 & 0.048 \\
  &  &   & &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &   &    & 
\\[-0.25cm]
  & OXY &  0.122 & 0.119 & 0.447 & \cellcolor{black!10}0.041 & \cellcolor{black!10}0.044 & \cellcolor{black!10}0.043 & 0.047 & 0.050 & 0.050 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Health Care}}} & JNJ & \cellcolor{black!10}0.052 & \cellcolor{black!10}0.037 & \cellcolor{black!10}0.041 & 0.508 & 0.100 & 0.089 & \cellcolor{black!10}0.055 & \cellcolor{black!10}0.044 & \cellcolor{black!10}0.065 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & LLY & \cellcolor{black!10}0.058 & \cellcolor{black!10}0.031 & \cellcolor{black!10}0.044 & 0.100 & 0.517 & 0.112 & \cellcolor{black!10}0.057 & \cellcolor{black!10}0.045 & \cellcolor{black!10}0.060 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & MRK & \cellcolor{black!10}0.053 & \cellcolor{black!10}0.034 & \cellcolor{black!10}0.043 & 0.089 & 0.112 & 0.486 & \cellcolor{black!10}0.057 & \cellcolor{black!10}0.051 & \cellcolor{black!10}0.055 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Info Tech.}}} & AAPL & 0.065 & 0.047 & 0.047 & \cellcolor{black!10}0.055 & \cellcolor{black!10}0.057 & \cellcolor{black!10}0.057 & 0.463 & 0.097 & 0.098 \\
  &  &  &   &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  & 
\\[-0.25cm]
  & MU &  0.062 & 0.043 & 0.050 & \cellcolor{black!10}0.044 & \cellcolor{black!10}0.045 & \cellcolor{black!10}0.051 & 0.097 & 0.462 & 0.093 \\
  &  &   &   &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  & & 
\\[-0.25cm]
  & ORCL &  0.064 & 0.048 & 0.050 & \cellcolor{black!10}0.065 & \cellcolor{black!10}0.060 & \cellcolor{black!10}0.055 & 0.098 & 0.093 & 0.487  \\
\\[0.0cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%(2)
 & & \multicolumn{9}{c}{\textit{Panel B: Asymmetric $B^\prime_{\rm{Chol}}$ Matrix by Group-$t$ Distribution}} \\
\\[-0.2cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Energy}}} & CVX & 0.401 & 0.000 & 0.000 & \cellcolor{black!10}0.083 & \cellcolor{black!10}0.000 & \cellcolor{black!10}0.000 & 0.250 & 0.000 & 0.000 \\
  &  &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &   &  
\\[-0.25cm]
  & MRO & 0.187 & 0.389 & 0.000 & \cellcolor{black!10}0.073 & \cellcolor{black!10}0.012 & \cellcolor{black!10}0.000 & 0.190 & 0.015 & 0.000 \\
  &  &   & &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &   &    & 
\\[-0.25cm]
  & OXY &  0.228 & 0.135 & 0.375 & \cellcolor{black!10}0.080 & \cellcolor{black!10}0.000 & \cellcolor{black!10}0.011 & 0.155 & 0.017 & 0.019 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Health Care}}} & JNJ & \cellcolor{black!10}0.261 & \cellcolor{black!10}0.087 & \cellcolor{black!10}0.052 & -0.382 & 0.041 & 0.252 & \cellcolor{black!10}0.021 & \cellcolor{black!10}-0.013 & \cellcolor{black!10}0.007  \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & LLY & \cellcolor{black!10}0.262 & \cellcolor{black!10}0.077 & \cellcolor{black!10}0.047 & -0.191 & -0.436 & -0.023 & \cellcolor{black!10}-0.016 & \cellcolor{black!10}-0.024 & \cellcolor{black!10}0.016  \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & MRK & \cellcolor{black!10}0.256 & \cellcolor{black!10}0.076 & \cellcolor{black!10}0.067 & -0.306 & 0.012 & -0.319 & \cellcolor{black!10}0.007 & \cellcolor{black!10}0.001 & \cellcolor{black!10}0.004 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Info Tech.}}} & AAPL & 0.340 & 0.110 & 0.017 & \cellcolor{black!10}0.046 & \cellcolor{black!10}0.034 & \cellcolor{black!10}-0.001 & -0.200 & -0.144 & 0.244 \\
  &  &  &   &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  & 
\\[-0.25cm]
  & MU &   0.317 & 0.081 & 0.022 & \cellcolor{black!10}0.039 & \cellcolor{black!10}0.013 & \cellcolor{black!10}0.004 & -0.178 & 0.324 & 0.029 \\
  &  &   &   &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  & & 
\\[-0.25cm]
  & ORCL &  0.349 & 0.114 & 0.048 & \cellcolor{black!10}0.031 & \cellcolor{black!10}0.018 & \cellcolor{black!10}0.018 & -0.202 & -0.111 & -0.287  \\
\\[0.0cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%(3)
 & & \multicolumn{9}{c}{\textit{Panel C: Asymmetric $B^\prime$ Matrix by Hetero-$t$ Distribution}} \\
\\[-0.2cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Energy}}} & CVX & \cellcolor{black!10}0.365 & -0.114 & -0.098 & -0.045 & -0.026 & -0.065 & -0.243 & -0.049 & -0.077 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  &  &  &   &  
\\[-0.25cm]
  & MRO & \cellcolor{black!10}0.307 & \cellcolor{black!10}0.304 & 0.033 & -0.037 & -0.022 & -0.057 & -0.180 & -0.021 & -0.050  \\
  &  &  \cellcolor{black!10} & & \cellcolor{black!10} & &  & &   &    & 
\\[-0.25cm]
  & OXY &  \cellcolor{black!10}0.314 & -0.042 & \cellcolor{black!10}0.328 & -0.042 & -0.019 & -0.057 & -0.152 & -0.018 & -0.072 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Health Care}}} & JNJ & \cellcolor{black!10}0.282 & -0.017 & 0.003 & \cellcolor{black!10}0.446 & 0.055 & 0.093 & 0.000 & -0.015 & -0.011 \\
  &  & \cellcolor{black!10} &  & &  &\cellcolor{black!10}  &   &  &  &
\\[-0.25cm]
  & LLY & \cellcolor{black!10}0.291 & -0.035 & -0.012 & 0.027 & \cellcolor{black!10}0.459 & 0.071 & 0.039 & -0.036 & 0.002 \\
  &  & \cellcolor{black!10} &  &  &  &  & \cellcolor{black!10} &  &  & 
\\[-0.25cm]
  & MRK & \cellcolor{black!10}0.281 & -0.021 & 0.002 & -0.019 & 0.052 & \cellcolor{black!10}0.434 & -0.010 & -0.008 & -0.002 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Info Tech.}}} & AAPL & \cellcolor{black!10}0.360 & -0.009 & -0.042 & -0.035 & -0.070 & -0.032 & \cellcolor{black!10}0.281 & -0.123 & -0.139 \\
  &  & \cellcolor{black!10} &   &  &  &  &  &  & \cellcolor{black!10} & 
\\[-0.25cm]
  & MU &   \cellcolor{black!10}0.329 & -0.033 & -0.034 & -0.031 & -0.029 & -0.031 & 0.118 & \cellcolor{black!10}0.346 & -0.005 \\
  &  &  \cellcolor{black!10} &   &   &  & &  &  & & \cellcolor{black!10}
\\[-0.25cm]
  & ORCL &  \cellcolor{black!10}0.364 & -0.028 & -0.007 & -0.005 & -0.045 & -0.036 & 0.097 & -0.054 & \cellcolor{black!10}0.355  \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/Table51.tex <==
\vspace{0.2cm}
\begin{small}
%\begin{tabular}{p{0.3cm}  p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} }
\begin{tabularx}{\textwidth}{m{0.5cm}XYYYYYYYYY}
\toprule
\midrule
  & &  \multicolumn{3}{c}{Energy} & \multicolumn{3}{c}{Health Care} & \multicolumn{3}{c}{Information Tech.} \\
\cmidrule(l){3-5}
\cmidrule(l){6-8}
\cmidrule(l){9-11}
  &  & CVX & MRO & OXY   & JNJ   & LLY   & MRK & AAPL & MU & ORCL \\
\midrule
 & & \multicolumn{9}{c}{\textit{Panel A: Symmetric $B^\prime$ Matrix from $\hat{\Sigma}^{\frac{1}{2}}$}} \\
\\[-0.2cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad  Energy}}} & CVX & 0.425 & 0.116 & 0.122 & \cellcolor{black!10}0.052 & \cellcolor{black!10}0.058 & \cellcolor{black!10}0.053 & 0.065 & 0.062 & 0.064 \\
  &  &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &   &  
\\[-0.25cm]
  & MRO & 0.116 & 0.437 & 0.119 & \cellcolor{black!10}0.037 & \cellcolor{black!10}0.031 & \cellcolor{black!10}0.034 & 0.047 & 0.043 & 0.048 \\
  &  &   & &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &   &    & 
\\[-0.25cm]
  & OXY &  0.122 & 0.119 & 0.447 & \cellcolor{black!10}0.041 & \cellcolor{black!10}0.044 & \cellcolor{black!10}0.043 & 0.047 & 0.050 & 0.050 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Health Care}}} & JNJ & \cellcolor{black!10}0.052 & \cellcolor{black!10}0.037 & \cellcolor{black!10}0.041 & 0.508 & 0.100 & 0.089 & \cellcolor{black!10}0.055 & \cellcolor{black!10}0.044 & \cellcolor{black!10}0.065 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & LLY & \cellcolor{black!10}0.058 & \cellcolor{black!10}0.031 & \cellcolor{black!10}0.044 & 0.100 & 0.517 & 0.112 & \cellcolor{black!10}0.057 & \cellcolor{black!10}0.045 & \cellcolor{black!10}0.060 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & MRK & \cellcolor{black!10}0.053 & \cellcolor{black!10}0.034 & \cellcolor{black!10}0.043 & 0.089 & 0.112 & 0.486 & \cellcolor{black!10}0.057 & \cellcolor{black!10}0.051 & \cellcolor{black!10}0.055 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Info Tech.}}} & AAPL & 0.065 & 0.047 & 0.047 & \cellcolor{black!10}0.055 & \cellcolor{black!10}0.057 & \cellcolor{black!10}0.057 & 0.463 & 0.097 & 0.098 \\
  &  &  &   &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  & 
\\[-0.25cm]
  & MU &  0.062 & 0.043 & 0.050 & \cellcolor{black!10}0.044 & \cellcolor{black!10}0.045 & \cellcolor{black!10}0.051 & 0.097 & 0.462 & 0.093 \\
  &  &   &   &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  & & 
\\[-0.25cm]
  & ORCL &  0.064 & 0.048 & 0.050 & \cellcolor{black!10}0.065 & \cellcolor{black!10}0.060 & \cellcolor{black!10}0.055 & 0.098 & 0.093 & 0.487  \\
\\[0.0cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%(2)
 & & \multicolumn{9}{c}{\textit{Panel B: Asymmetric $B^\prime$ Matrix by Group-$t$ Distribution}} \\
\\[-0.2cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Energy}}} & CVX & 0.373 & 0.092 & 0.117 & \cellcolor{black!10}-0.063 & \cellcolor{black!10}-0.020 & \cellcolor{black!10}-0.050 & -0.155 & -0.125 & -0.151 \\
  &  &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &   &  
\\[-0.25cm]
  & MRO & 0.066 & 0.412 & 0.111 & \cellcolor{black!10}-0.053 & \cellcolor{black!10}-0.030 & \cellcolor{black!10}-0.042 & -0.124 & -0.081 & -0.120 \\
  &  &   & &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &   &    & 
\\[-0.25cm]
  & OXY &  0.083 & 0.099 & 0.440 & \cellcolor{black!10}-0.054 & \cellcolor{black!10}-0.020 & \cellcolor{black!10}-0.056 & -0.090 & -0.061 & -0.113 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Health Care}}} & JNJ & \cellcolor{black!10}0.206 & \cellcolor{black!10}0.131 & \cellcolor{black!10}0.137 & 0.455 & 0.052 & 0.039 & \cellcolor{black!10}-0.003 & \cellcolor{black!10}-0.021 & \cellcolor{black!10}-0.014 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & LLY & \cellcolor{black!10}0.210 & \cellcolor{black!10}0.123 & \cellcolor{black!10}0.132 & 0.049 & 0.469 & 0.064 & \cellcolor{black!10}0.030 & \cellcolor{black!10}-0.012 & \cellcolor{black!10}0.005 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10}
\\[-0.25cm]
  & MRK & \cellcolor{black!10}0.200 & \cellcolor{black!10}0.116 & \cellcolor{black!10}0.148 & 0.037 & 0.065 & 0.436 & \cellcolor{black!10}-0.002 & \cellcolor{black!10}-0.002 & \cellcolor{black!10}-0.007 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Info Tech.}}} & AAPL & 0.281 & 0.179 & 0.131 & \cellcolor{black!10}-0.029 & \cellcolor{black!10}-0.044 & \cellcolor{black!10}-0.022 & 0.346 & -0.007 & -0.017 \\
  &  &  &   &  & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  &  & 
\\[-0.25cm]
  & MU &   0.267 & 0.145 & 0.125 & \cellcolor{black!10}-0.025 & \cellcolor{black!10}-0.022 & \cellcolor{black!10}-0.024 & -0.004 & 0.371 & -0.008 \\
  &  &   &   &   & \cellcolor{black!10} & \cellcolor{black!10} & \cellcolor{black!10} &  & & 
\\[-0.25cm]
  & ORCL &  0.281 & 0.178 & 0.163 & \cellcolor{black!10}-0.009 & \cellcolor{black!10}-0.025 & \cellcolor{black!10}-0.030 & -0.021 & -0.015 & 0.368  \\
\\[0.0cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%(3)
 & & \multicolumn{9}{c}{\textit{Panel C: Asymmetric $B^\prime$ Matrix by Hetero-$t$ Distribution}} \\
\\[-0.2cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Energy}}} & CVX & \cellcolor{black!10}0.365 & -0.114 & -0.098 & -0.045 & -0.026 & -0.065 & -0.243 & -0.049 & -0.077 \\
  &  & \cellcolor{black!10} & \cellcolor{black!10} &  &  &  &  &  &   &  
\\[-0.25cm]
  & MRO & \cellcolor{black!10}0.307 & \cellcolor{black!10}0.304 & 0.033 & -0.037 & -0.022 & -0.057 & -0.180 & -0.021 & -0.050  \\
  &  &  \cellcolor{black!10} & & \cellcolor{black!10} & &  & &   &    & 
\\[-0.25cm]
  & OXY &  \cellcolor{black!10}0.314 & -0.042 & \cellcolor{black!10}0.328 & -0.042 & -0.019 & -0.057 & -0.152 & -0.018 & -0.072 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Health Care}}} & JNJ & \cellcolor{black!10}0.282 & -0.017 & 0.003 & \cellcolor{black!10}0.446 & 0.055 & 0.093 & 0.000 & -0.015 & -0.011 \\
  &  & \cellcolor{black!10} &  & &  &\cellcolor{black!10}  &   &  &  &
\\[-0.25cm]
  & LLY & \cellcolor{black!10}0.291 & -0.035 & -0.012 & 0.027 & \cellcolor{black!10}0.459 & 0.071 & 0.039 & -0.036 & 0.002 \\
  &  & \cellcolor{black!10} &  &  &  &  & \cellcolor{black!10} &  &  & 
\\[-0.25cm]
  & MRK & \cellcolor{black!10}0.281 & -0.021 & 0.002 & -0.019 & 0.052 & \cellcolor{black!10}0.434 & -0.010 & -0.008 & -0.002 \\
\\[-0.25cm]
 \parbox[c]{1cm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize \quad Info Tech.}}} & AAPL & \cellcolor{black!10}0.360 & -0.009 & -0.042 & -0.035 & -0.070 & -0.032 & \cellcolor{black!10}0.281 & -0.123 & -0.139 \\
  &  & \cellcolor{black!10} &   &  &  &  &  &  & \cellcolor{black!10} & 
\\[-0.25cm]
  & MU &   \cellcolor{black!10}0.329 & -0.033 & -0.034 & -0.031 & -0.029 & -0.031 & 0.118 & \cellcolor{black!10}0.346 & -0.005 \\
  &  &  \cellcolor{black!10} &   &   &  & &  &  & & \cellcolor{black!10}
\\[-0.25cm]
  & ORCL &  \cellcolor{black!10}0.364 & -0.028 & -0.007 & -0.005 & -0.045 & -0.036 & 0.097 & -0.054 & \cellcolor{black!10}0.355  \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/TableSimulation_ASym.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{1.3cm}Yp{-0.2cm}YYYp{-0.2cm}YYYY}
\toprule
\midrule
          & {True} &       & Mean   & Std   & aStd  &       & Mean   & Std   & aStd \\
\midrule
          &   &  &  \multicolumn{3}{c}{$T=500$}     &       & \multicolumn{3}{c}{$T=1,000$} \\
\\[-0.2cm]          
    $\mu_1$   & 0.1000 &       & 0.1000 & 0.0337 & 0.0339 &       & 0.1003 & 0.0237 & 0.0239 \\
\\[-0.35cm]  
    $\mu_2$   & 0.2000 &       & 0.2000 & 0.0480 & 0.0484 &       & 0.2004 & 0.0338 & 0.0342 \\
\\[-0.35cm] 
    $\mu_3$   & 0.3000 &       & 0.3001 & 0.0604 & 0.0609 &       & 0.3004 & 0.0427 & 0.0431 \\
\\[-0.35cm] 
    $1/\nu_1$    & 0.2500 &       & 0.2496 & 0.0340 & 0.0335 &       & 0.2497 & 0.0235 & 0.0237 \\
\\[-0.35cm] 
    $1/\nu_2$    & 0.1250 &       & 0.1222 & 0.0433 & 0.0413 &       & 0.1240 & 0.0299 & 0.0292 \\
\\[-0.35cm] 
    \multirow{6}[0]{*}{$\rm{vech}(\Omega_1)$} & 0.1000 &       & 0.1023 & 0.0258 & 0.0232 &       & 0.1012 & 0.0174 & 0.0164 \\
\\[-0.35cm] 
          & 0.1700 &       & 0.1729 & 0.0397 & 0.0360 &       & 0.1715 & 0.0269 & 0.0254 \\
\\[-0.35cm] 
          & 0.2500 &       & 0.2529 & 0.0536 & 0.0489 &       & 0.2517 & 0.0364 & 0.0345 \\
\\[-0.35cm] 
          & 0.2900 &       & 0.2935 & 0.0607 & 0.0553 &       & 0.2919 & 0.0412 & 0.0391 \\
\\[-0.35cm] 
          & 0.4300 &       & 0.4334 & 0.0816 & 0.0749 &       & 0.4321 & 0.0555 & 0.0529 \\
\\[-0.35cm] 
          & 0.6500 &       & 0.6529 & 0.1095 & 0.1014 &       & 0.6521 & 0.0748 & 0.0717 \\
\\[-0.35cm] 
    \multirow{6}[0]{*}{$\rm{vech}(\Omega_2)$} & 0.3600 &       & 0.3584 & 0.0493 & 0.0464 &       & 0.3589 & 0.0335 & 0.0328 \\
\\[-0.35cm] 
          & 0.4800 &       & 0.4781 & 0.0693 & 0.0649 &       & 0.4786 & 0.0470 & 0.0459 \\
\\[-0.35cm] 
          & 0.5400 &       & 0.5383 & 0.0843 & 0.0786 &       & 0.5385 & 0.0570 & 0.0556 \\
\\[-0.35cm] 
          & 0.6400 &       & 0.6379 & 0.0975 & 0.0910 &       & 0.6383 & 0.0659 & 0.0643 \\
\\[-0.35cm] 
          & 0.7200 &       & 0.7184 & 0.1188 & 0.1103 &       & 0.7183 & 0.0800 & 0.0780 \\
\\[-0.35cm] 
          & 0.8100 &       & 0.8093 & 0.1449 & 0.1341 &       & 0.8084 & 0.0974 & 0.0948 \\
\\[0.0cm]
          &  &    & \multicolumn{3}{c}{$T=2,000$}     &       & \multicolumn{3}{c}{$T=5,000$} \\
\\[-0.2cm]
    $\mu_1$   & 0.1000 &       & 0.1003 & 0.0169 & 0.0169 &       & 0.1000 & 0.0107 & 0.0107 \\
\\[-0.35cm]
    $\mu_2$   & 0.2000 &       & 0.2004 & 0.0242 & 0.0242 &       & 0.2000 & 0.0152 & 0.0153 \\
\\[-0.35cm]
    $\mu_3$   & 0.3000 &       & 0.3004 & 0.0305 & 0.0305 &       & 0.3001 & 0.0192 & 0.0193 \\
\\[-0.35cm]
    $1/\nu_1$    & 0.2500 &       & 0.2498 & 0.0166 & 0.0168 &       & 0.2499 & 0.0106 & 0.0106 \\
\\[-0.35cm]
    $1/\nu_2$    & 0.1250 &       & 0.1241 & 0.0211 & 0.0206 &       & 0.1248 & 0.0130 & 0.0130 \\
\\[-0.35cm]
    \multirow{6}[0]{*}{$\rm{vech}(\Omega_1)$} & 0.1000 &       & 0.1006 & 0.0118 & 0.0116 &       & 0.1003 & 0.0075 & 0.0073 \\
\\[-0.35cm]
          & 0.1700 &       & 0.1708 & 0.0182 & 0.0180 &       & 0.1704 & 0.0115 & 0.0114 \\
\\[-0.35cm]
          & 0.2500 &       & 0.2509 & 0.0247 & 0.0244 &       & 0.2505 & 0.0157 & 0.0154 \\
\\[-0.35cm]
          & 0.2900 &       & 0.2911 & 0.0280 & 0.0277 &       & 0.2906 & 0.0177 & 0.0175 \\
\\[-0.35cm]
          & 0.4300 &       & 0.4313 & 0.0378 & 0.0374 &       & 0.4306 & 0.0240 & 0.0237 \\
\\[-0.35cm]
          & 0.6500 &       & 0.6515 & 0.0512 & 0.0507 &       & 0.6507 & 0.0323 & 0.0321 \\
\\[-0.35cm]
    \multirow{6}[0]{*}{$\rm{vech}(\Omega_2)$} & 0.3600 &       & 0.3597 & 0.0236 & 0.0232 &       & 0.3597 & 0.0146 & 0.0147 \\
\\[-0.35cm]
          & 0.4800 &       & 0.4796 & 0.0330 & 0.0325 &       & 0.4796 & 0.0205 & 0.0205 \\
\\[-0.35cm]
          & 0.5400 &       & 0.5395 & 0.0400 & 0.0393 &       & 0.5396 & 0.0248 & 0.0249 \\
\\[-0.35cm]
          & 0.6400 &       & 0.6395 & 0.0463 & 0.0455 &       & 0.6395 & 0.0287 & 0.0288 \\
\\[-0.35cm]
          & 0.7200 &       & 0.7195 & 0.0561 & 0.0552 &       & 0.7195 & 0.0348 & 0.0349 \\
\\[-0.35cm]
          & 0.8100 &       & 0.8095 & 0.0682 & 0.0670 &       & 0.8094 & 0.0424 & 0.0424 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/TableSimulation_SPX.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{1.3cm}Yp{-0.2cm}YYYp{-0.2cm}YYYY}
\toprule
\midrule
          & {True} &       & Mean   & Std   & aStd  &       & Mean   & Std   & aStd \\
\midrule
          &   &  &  \multicolumn{3}{c}{$T=500$}     &       & \multicolumn{3}{c}{$T=1,000$} \\
\\[-0.2cm]          
    $\mu_1$   & 0.1000 &       & 0.1011 & 0.0715 & 0.0716 &       & 0.1004 & 0.0506 & 0.0506 \\
    $\mu_2$   & 0.2000 &       & 0.2016 & 0.0819 & 0.0823 &       & 0.2005 & 0.0586 & 0.0582 \\
    $\mu_3$   & 0.3000 &       & 0.3017 & 0.0802 & 0.0806 &       & 0.3006 & 0.0575 & 0.0570 \\
    $\mu_4$   & 0.4000 &       & 0.4019 & 0.0960 & 0.0967 &       & 0.4006 & 0.0690 & 0.0683 \\
    \multirow{16}[0]{*}{$\rm{vec}(\Xi)$} & 0.1000 &       & 0.1172 & 0.0557 & 0.0568 &       & 0.1082 & 0.0389 & 0.0402 \\
          & 0.2000 &       & 0.2018 & 0.0739 & 0.0681 &       & 0.2005 & 0.0501 & 0.0481 \\
          & 0.3000 &       & 0.2916 & 0.0863 & 0.0810 &       & 0.2956 & 0.0575 & 0.0573 \\
          & 0.4000 &       & 0.3903 & 0.1013 & 0.0939 &       & 0.3949 & 0.0673 & 0.0664 \\
          & 0.2000 &       & 0.2018 & 0.0739 & 0.0681 &       & 0.2005 & 0.0501 & 0.0481 \\
          & 0.5000 &       & 0.5003 & 0.0795 & 0.0707 &       & 0.4998 & 0.0529 & 0.0500 \\
          & 0.6000 &       & 0.6033 & 0.0719 & 0.0672 &       & 0.6013 & 0.0483 & 0.0475 \\
          & 0.7000 &       & 0.7064 & 0.0837 & 0.0808 &       & 0.7028 & 0.0570 & 0.0572 \\
          & 0.8000 &       & 0.7959 & 0.0494 & 0.0467 &       & 0.7984 & 0.0338 & 0.0330 \\
          & 0.9000 &       & 0.8957 & 0.0526 & 0.0500 &       & 0.8983 & 0.0358 & 0.0354 \\
          & 1.0000 &       & 0.9946 & 0.0548 & 0.0518 &       & 0.9976 & 0.0369 & 0.0366 \\
          & 1.1000 &       & 1.0940 & 0.0641 & 0.0607 &       & 1.0974 & 0.0432 & 0.0429 \\
          & 1.2000 &       & 1.1929 & 0.0554 & 0.0531 &       & 1.1969 & 0.0374 & 0.0375 \\
          & 1.3000 &       & 1.2929 & 0.0645 & 0.0615 &       & 1.2971 & 0.0435 & 0.0435 \\
          & 1.1000 &       & 1.0940 & 0.0641 & 0.0607 &       & 1.0974 & 0.0432 & 0.0429 \\
          & 1.4000 &       & 1.3916 & 0.0780 & 0.0739 &       & 1.3964 & 0.0527 & 0.0523 \\
    $1/\nu_1$  & 0.2500 &       & 0.2514 & 0.0341 & 0.0335 &       & 0.2508 & 0.0241 & 0.0237 \\
    $1/\nu_2$  & 0.1250 &       & 0.1240 & 0.0291 & 0.0280 &       & 0.1249 & 0.0202 & 0.0198 \\
          &       &       &       &       &       &       &       &       &  \\
          &  &    & \multicolumn{3}{c}{$T=2,000$}     &       & \multicolumn{3}{c}{$T=5,000$} \\
\\[-0.2cm]
    $\mu_1$   & 0.1000 &       & 0.0998 & 0.0359 & 0.0358 &       & 0.0999 & 0.0229 & 0.0226 \\
    $\mu_2$   & 0.2000 &       & 0.1999 & 0.0413 & 0.0412 &       & 0.1999 & 0.0262 & 0.0260 \\
    $\mu_3$   & 0.3000 &       & 0.3000 & 0.0404 & 0.0403 &       & 0.2999 & 0.0256 & 0.0255 \\
    $\mu_4$   & 0.4000 &       & 0.4000 & 0.0485 & 0.0483 &       & 0.3998 & 0.0307 & 0.0306 \\
    \multirow{16}[0]{*}{$\rm{vec}(\Xi)$} & 0.1000 &       & 0.1037 & 0.0274 & 0.0284 &       & 0.1008 & 0.0175 & 0.0180 \\
          & 0.2000 &       & 0.2000 & 0.0349 & 0.0340 &       & 0.1998 & 0.0216 & 0.0215 \\
          & 0.3000 &       & 0.2977 & 0.0405 & 0.0405 &       & 0.2992 & 0.0256 & 0.0256 \\
          & 0.4000 &       & 0.3973 & 0.0473 & 0.0470 &       & 0.3989 & 0.0297 & 0.0297 \\
          & 0.2000 &       & 0.2000 & 0.0349 & 0.0340 &       & 0.1998 & 0.0216 & 0.0215 \\
          & 0.5000 &       & 0.4997 & 0.0364 & 0.0354 &       & 0.4993 & 0.0226 & 0.0224 \\
          & 0.6000 &       & 0.6005 & 0.0334 & 0.0336 &       & 0.5994 & 0.0212 & 0.0213 \\
          & 0.7000 &       & 0.7012 & 0.0397 & 0.0404 &       & 0.6995 & 0.0253 & 0.0256 \\
          & 0.8000 &       & 0.7987 & 0.0234 & 0.0233 &       & 0.7999 & 0.0147 & 0.0148 \\
          & 0.9000 &       & 0.8988 & 0.0253 & 0.0250 &       & 0.8999 & 0.0157 & 0.0158 \\
          & 1.0000 &       & 0.9986 & 0.0263 & 0.0259 &       & 0.9997 & 0.0162 & 0.0164 \\
          & 1.1000 &       & 1.0984 & 0.0309 & 0.0303 &       & 1.0997 & 0.0190 & 0.0192 \\
          & 1.2000 &       & 1.1982 & 0.0270 & 0.0265 &       & 1.1993 & 0.0165 & 0.0168 \\
          & 1.3000 &       & 1.2981 & 0.0313 & 0.0308 &       & 1.2995 & 0.0192 & 0.0194 \\
          & 1.1000 &       & 1.0984 & 0.0309 & 0.0303 &       & 1.0997 & 0.0190 & 0.0192 \\
          & 1.4000 &       & 1.3978 & 0.0376 & 0.0369 &       & 1.3996 & 0.0231 & 0.0234 \\
   $1/\nu_1$  & 0.2500 &       & 0.2501 & 0.0166 & 0.0168 &       & 0.2502 & 0.0107 & 0.0106 \\
   $1/\nu_2$  & 0.1250 &       & 0.1247 & 0.0141 & 0.0140 &       & 0.1247 & 0.0088 & 0.0088 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/TableSimulation_SPX2.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{1.3cm}Yp{-0.2cm}YYYp{-0.2cm}YYYY}
\toprule
\midrule
          & {True} &       & Mean   & Std   & aStd  &       & Mean   & Std   & aStd \\
\midrule
          &   &  &  \multicolumn{3}{c}{$T=500$}     &       & \multicolumn{3}{c}{$T=1,000$} \\
\\[-0.2cm] 
    $\mu_1$   & 0.1000 &       & 0.1000 & 0.0396 & 0.0398 &       & 0.0999 & 0.0280 & 0.0282 \\
    $\mu_2$   & 0.2000 &       & 0.2000 & 0.0396 & 0.0397 &       & 0.1999 & 0.0278 & 0.0281 \\
    $\mu_3$   & 0.3000 &       & 0.3000 & 0.0515 & 0.0515 &       & 0.2999 & 0.0361 & 0.0364 \\
    \multirow{9}[0]{*}{$\rm{vec}(\Xi)$} & 0.1000 &       & 0.1003 & 0.0501 & 0.0463 &       & 0.0998 & 0.0349 & 0.0327 \\
          & 0.2000 &       & 0.1994 & 0.0496 & 0.0459 &       & 0.1994 & 0.0344 & 0.0324 \\
          & 0.3000 &       & 0.2990 & 0.0640 & 0.0594 &       & 0.2991 & 0.0445 & 0.0420 \\
          & 0.4000 &       & 0.3989 & 0.0230 & 0.0223 &       & 0.3993 & 0.0159 & 0.0158 \\
          & 0.5000 &       & 0.4986 & 0.0231 & 0.0226 &       & 0.4991 & 0.0161 & 0.0160 \\
          & 0.6000 &       & 0.5985 & 0.0299 & 0.0292 &       & 0.5990 & 0.0208 & 0.0206 \\
          & 0.7000 &       & 0.6980 & 0.0302 & 0.0297 &       & 0.6987 & 0.0210 & 0.0210 \\
          & 0.6000 &       & 0.5985 & 0.0299 & 0.0292 &       & 0.5990 & 0.0208 & 0.0206 \\
          & 0.8000 &       & 0.7978 & 0.0400 & 0.0390 &       & 0.7986 & 0.0279 & 0.0275 \\
    $1/\nu_1$  & 0.2500 &       & 0.2496 & 0.0474 & 0.0463 &       & 0.2495 & 0.0330 & 0.0327 \\
    $1/\nu_2$  & 0.1250 &       & 0.1236 & 0.0285 & 0.0280 &       & 0.1244 & 0.0200 & 0.0198 \\
          &       &       &       &       &       &       &       &       &  \\
          &  &    & \multicolumn{3}{c}{$T=2,000$}     &       & \multicolumn{3}{c}{$T=5,000$} \\
\\[-0.2cm]
    $\mu_1$   & 0.1000 &       & 0.1000 & 0.0199 & 0.0199 &       & 0.1002 & 0.0126 & 0.0126 \\
    $\mu_2$   & 0.2000 &       & 0.2000 & 0.0198 & 0.0198 &       & 0.2002 & 0.0126 & 0.0126 \\
    $\mu_3$   & 0.3000 &       & 0.3000 & 0.0258 & 0.0257 &       & 0.3003 & 0.0163 & 0.0163 \\
    \multirow{9}[0]{*}{$\rm{vec}(\Xi)$} & 0.1000 &       & 0.0992 & 0.0240 & 0.0231 &       & 0.1000 & 0.0151 & 0.0146 \\
          & 0.2000 &       & 0.1990 & 0.0238 & 0.0229 &       & 0.2000 & 0.0150 & 0.0145 \\
          & 0.3000 &       & 0.2987 & 0.0308 & 0.0297 &       & 0.2999 & 0.0194 & 0.0188 \\
          & 0.4000 &       & 0.3998 & 0.0113 & 0.0112 &       & 0.3999 & 0.0070 & 0.0071 \\
          & 0.5000 &       & 0.4997 & 0.0114 & 0.0113 &       & 0.4999 & 0.0071 & 0.0072 \\
          & 0.6000 &       & 0.5997 & 0.0147 & 0.0146 &       & 0.5999 & 0.0092 & 0.0092 \\
          & 0.7000 &       & 0.6995 & 0.0149 & 0.0148 &       & 0.6999 & 0.0093 & 0.0094 \\
          & 0.6000 &       & 0.5997 & 0.0147 & 0.0146 &       & 0.5999 & 0.0092 & 0.0092 \\
          & 0.8000 &       & 0.7997 & 0.0197 & 0.0195 &       & 0.7998 & 0.0123 & 0.0123 \\
    $1/\nu_1$  & 0.2500 &       & 0.2500 & 0.0232 & 0.0232 &       & 0.2500 & 0.0147 & 0.0146 \\
    $1/\nu_2$  & 0.1250 &       & 0.1248 & 0.0142 & 0.0140 &       & 0.1249 & 0.0088 & 0.0088 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}

==> Tables/TableSimulation_Sym.tex <==
\vspace{0.2cm}
\begin{small}
\begin{tabularx}{\textwidth}{p{0.7cm}YYYYYp{-0.2cm}YYYYYYYY}
\toprule
\midrule
          & {True} & Mean  & Bias  & Std   & aStd  &       & Mean  & Bias  & Std   & aStd \\
\midrule
          &       \multicolumn{5}{c}{$T=100$}     &       & \multicolumn{4}{c}{$T=500$} \\
\\[-0.2cm]          
    $\mu_1$   & 1     & 1.0015 & 0.0015 & 0.6218 & 0.6137 &       & 0.9974 & -0.0026 & 0.2737 & 0.2745 \\
\\[-0.35cm]
    $\mu_2$   & 2     & 1.9947 & -0.0053 & 0.9223 & 0.9159 &       & 1.9970 & -0.0030 & 0.4077 & 0.4096 \\
\\[-0.35cm]
    $\mu_3$   & 3     & 2.9997 & -0.0003 & 1.1178 & 1.1116 &       & 2.9968 & -0.0032 & 0.4940 & 0.4971 \\
\\[-0.35cm]
    $B^{\prime}_{11}$  & 4     & 3.9989 & -0.0011 & 0.3753 & 0.3615 &       & 4.0032 & 0.0032 & 0.1641 & 0.1617 \\
\\[-0.35cm]
    $B^{\prime}_{21}$  & 2     & 2.0025 & 0.0025 & 0.2983 & 0.2891 &       & 2.0052 & 0.0052 & 0.1324 & 0.1293 \\
\\[-0.35cm]
    $B^{\prime}_{31}$  & 3     & 3.0049 & 0.0049 & 0.3479 & 0.3367 &       & 3.0058 & 0.0058 & 0.1541 & 0.1506 \\
\\[-0.35cm]
    $B^{\prime}_{22}$  & 6     & 6.0050 & 0.0050 & 0.5498 & 0.5272 &       & 6.0078 & 0.0078 & 0.2391 & 0.2358 \\
\\[-0.35cm]
    $B^{\prime}_{32}$  & 5     & 5.0077 & 0.0077 & 0.5196 & 0.5015 &       & 5.0097 & 0.0097 & 0.2276 & 0.2243 \\
\\[-0.35cm]
    $B^{\prime}_{33}$  & 8     & 8.0040 & 0.0040 & 0.7582 & 0.7365 &       & 8.0155 & 0.0155 & 0.3367 & 0.3294 \\
\\[-0.35cm]
    $1/\nu_1$  & 1/4  & 0.2403 & -0.0097 & 0.0806 & 0.0744 &       & 0.2475 & -0.0025 & 0.0337 & 0.0333 \\
\\[-0.35cm]
    $1/\nu_2$  & 1/8 & 0.1125 & -0.0125 & 0.0891 & 0.0901 &       & 0.1206 & -0.0044 & 0.0418 & 0.0403 \\
          &       &       &       &       &       &       &       &       &       &  \\
          &        \multicolumn{5}{c}{$T=1,000$}    &       & \multicolumn{4}{c}{$T=5,000$} \\
\\[-0.2cm]
    $\mu_1$   & 1     & 1.0008 & 0.0008 & 0.1942 & 0.1941 &       & 0.9996 & -0.0004 & 0.0878 & 0.0868 \\
\\[-0.35cm]
    $\mu_2$   & 2     & 2.0040 & 0.0040 & 0.2904 & 0.2896 &       & 2.0007 & 0.0007 & 0.1305 & 0.1295 \\
\\[-0.35cm]
    $\mu_3$   & 3     & 3.0023 & 0.0023 & 0.3527 & 0.3515 &       & 3.0006 & 0.0006 & 0.1586 & 0.1572 \\
\\[-0.35cm]
    $B^{\prime}_{11}$  & 4     & 4.0012 & 0.0012 & 0.1151 & 0.1143 &       & 4.0001 & 0.0001 & 0.0514 & 0.0511 \\
\\[-0.35cm]
    $B^{\prime}_{21}$  & 2     & 2.0019 & 0.0019 & 0.0901 & 0.0914 &       & 2.0000 & 0.0000 & 0.0411 & 0.0409 \\
\\[-0.35cm]
    $B^{\prime}_{31}$  & 3     & 3.0032 & 0.0032 & 0.1059 & 0.1065 &       & 3.0000 & 0.0000 & 0.0481 & 0.0476 \\
\\[-0.35cm]
    $B^{\prime}_{22}$  & 6     & 6.0008 & 0.0008 & 0.1658 & 0.1667 &       & 6.0001 & 0.0001 & 0.0749 & 0.0746 \\
\\[-0.35cm]
    $B^{\prime}_{23}$  & 5    & 5.0034 & 0.0034 & 0.1574 & 0.1586 &       & 5.0000 & 0.0000 & 0.0708 & 0.0709 \\
\\[-0.35cm]
    $B^{\prime}_{33}$  & 8     & 8.0077 & 0.0077 & 0.2341 & 0.2329 &       & 8.0007 & 0.0007 & 0.1042 & 0.1042 \\
\\[-0.35cm]
    $1/\nu_1$  & 1/4  & 0.2490 & -0.0010 & 0.0236 & 0.0235 &       & 0.2498 & -0.0002 & 0.0106 & 0.0105 \\
\\[-0.35cm]
    $1/\nu_2$ & 1/8 & 0.1223 & -0.0027 & 0.0287 & 0.0285 &       & 0.1245 & -0.0005 & 0.0129 & 0.0127 \\
\\[0.0cm]
\\[-0.5cm]
\midrule
\bottomrule
\end{tabularx}
\end{small}
